Designing Multispecies Worlds for Robots, Cats, and Humans

We reflect on the design of a multispecies world centred around a bespoke enclosure in which three cats and a robot arm coexist for six hours a day during a twelve-day installation as part of an artist-led project. In this paper, we present the project's design process, encompassing various interconnected components, including the cats, the robot and its autonomous systems, the custom end-effectors and robot attachments, the diverse roles of the humans-in-the-loop, and the custom-designed enclosure. Subsequently, we provide a detailed account of key moments during the deployment and discuss the design implications for future multispecies systems. Specifically, we argue that designing the technology and its interactions is not sufficient, but that it is equally important to consider the design of the `world' in which the technology operates. Finally, we highlight the necessity of human involvement in areas such as breakdown recovery, animal welfare, and their role as audience.

==> Sections/X_Findings_3x3.tex <==
\section{Learnings}
Structure this around a 3x3 matrix.
Structure this around a 2x2 matrix.

What needs designing? What does `design' mean from different view points? Who are we designing for? 

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\hl{Maybe this table, or a generalisation of it that applies to other projects than Cat Royale, would be better fitted in the discussion?}
\begin{table}[H]
\begin{tabular}{l|p{4cm}p{4cm}p{4cm}}
& Environment & Movement & End-effectors / toys \\ \hline
\renewcommand{\arraystretch}{1.5}
Human & \textbullet~ How can we design an environment that is visually appealing for the audience? & \textbullet~ How can we design controllable moves for the robot operator? \newline \textbullet~ How can we design interesting moves for the audience? & \textbullet~ How can we design toys that are not to repetitive for the audience? \\ \hline

Robot & \textbullet~ How can we design an environment to allow the CV system to work efficiently? \newline \textbullet~ How can we guarantee safe robot operation through environment design? & \textbullet~ How can we design move sets that keep being engaging to the cats? & \textbullet~ How can we design end-effectors that support solid grabbing by the robot? \newline \textbullet~ How can we design end-effectors and toys that are robust enough for cats to engage with? \\ \hline

Cat & \textbullet~ How can we design a stimulating environment for the cats? \newline \textbullet~ How can we guarantee that the cats can withdraw consent through environmental design? & \textbullet~ How can we guarantee safe robot movement given the close proximity to the cats? \newline \textbullet~ How can we mimic real-life prey and play behaviour? & \textbullet~ How can we design end-effectors the cats can break? \newline \textbullet~ How can we design toys that provide sufficient variety?
\end{tabular}%
\caption{Example questions and dilemmas for each stakeholder and world design combination based on Cat Royale as a case. Multiple tensions arise as some of the interests are in opposition, e.g., an optimal environment for the CV based system might not be using a colour scheme that is visually appealing to either audience or cats, an acceptable compromise needs to be considered.}
\label{tab:my-table}
\end{table}

==> Sections/X_RobotAndWorld.tex <==
\subsection{The Robot and its World}
In order to investigate how an autonomous system, specifically an autonomous robotic system, could safely engage an audience while providing stimuli in a safe manner for cats, we needed to select a robot. However, this investigation: the research, design, safety considerations, aesthetics and the practical implementation of the 'world' required careful consideration. This was not only relevant for the selection of the specific robot, which in itself is part of the world, but also for the environment that it would co-inhabit with three cats. This section will highlight considerations that went into the robot and its design, as well as the context --- or world --- it was embedded in.

%In addition to the two types of actors (see~\Cref{sec:TheActors}) the design of Cat Royale required the design the robot as well as the world it would inhabit. 

\subsubsection{The Robot}\label{sec:TheRobot}
Just as the cat recruitment was vital, so was the selection of the robot used in the environment. The robot's morphology, range, movement speed, and lifting capacity provided, or stripped, the artist of different affordances in relation to the movements that could be executed. Furthermore, the robot, as instantiation of a physically embodied autonomous system, had a tangible impact on the cat well being and safety. For Cat Royale the emphasis was placed on using a lightweight robot with a small payload and reach, thereby allowing the cats to withdraw from the robot, which was vital to allow the cats to express contingent consent, without the need to leave the environment. The choice for the project fell on the Kinvoa Gen 3 Lite robot\footnote{https://www.kinovarobotics.com/product/gen3-lite-robots}, a small collaborative robot with .76 meters reach and a maximum payload of only .5 kg. However, with the robot in place, it became apparent that it was not sufficient as effective proxy between the artist and the cats. Several subsystems, \hl{both human and non-human}, needed to be put into place, and consecutively developed, in order to provide the artists with the possibility to implement their artistic vision. The robot (as part of a wider AI-based system) needed the capability to identify each individual cat and its position (utilising a computer vision system) and, following this, propose appropriate bespoke activities for each individual cat (using a decision engine), which aimed to maximise its happiness score. As part of the system the robot needed to be able to calculate a trajectory for the movement as well as safely execute it (robot operator).

%End-effectors 
With the robot selected, the next step was to provide it with affordances making it an effective proxy between artist and cats. These needed to allow it to manipulate a wide range of items (e.g., feathers, pillows, treats, or balls) in order to attempt to engage the cats. To provide the artists full artistic freedom, we choose to 3d design and print custom end-effectors. The customisation of end-effectors came with multiple advantages over relying on the standard 2-finger gripper, including easy and affordable access to prototyping different toys and movements, destructibility of the robot --- which allows the cats to, in some regard, overpower the robot --- and ease of expanding the toy repertoire available to the cats. Furthermore, the customisation allowed a wider range of of creative possibilities for the artists and enrichment activities for the cats.

%Movement
The, perhaps, most vital element about the robot was its movement. We needed to be able to generate movements with the robot that struck the perfect balance between predictable routine and exciting novelty for the cats. This was, however, not the only perspective on the robot movement, as the art installation needed to not only draw the cats, but also the audience in. While the installation started with a set of supported robot movements, the robot operator --- directed by the artists --- added new movements on a daily basis, ultimately increasing the capabilities of the robot. This daily need for the addition of new movements, necessitated the robot --- and its underlying systems --- to allow for rapid prototyping and development of new sequences. All movements were designed, tested, and finally implemented following the following mantra:

\begin{quote}
    \textit{``Design the robots movements in order to allow us to keep the cats engaged in a safe, but non-boring, way.''}
\end{quote}





%\begin{quote}
%    \hl{Note:} \textit{When does the artist/operator decide to overrule the decision engine and why? Who are we doing a favour, the cats, the robot, the audience, else?}
%\end{quote}

\subsubsection{The Robot World}
Inspired by art from the 70s, e.g., Verner Panton Visiona II exhibit\footnote{https://www.verner-panton.com/en/collection/visiona-2/}, Cat Royale's vision was to create a cat utopia using organic shapes and colours, which was of interest to and appropriate for the cats that would use the space, and of interest to the people who would be able to watch the cats in the space. The inspiration for the design of the environment focused upon supporting cat-centric needs, such as the presence of high perches and viewing-platforms, floor curvature which provides hiding places during prey-behaviour games with the robot, as well a soft --- and claw-able --- textures. The cats needs had to be aligned with the audience input, provided through the Audience Advisory Panel (AAP), the artists vision for the environment, as well as the animal welfare and behaviour experts expertise (i.e., a veterinarian as well as an expert in feline behaviour).

The environment went through numerous iterations, sketches, mock-ups, 3D renderings, physical scale models, until the final design was installed (see~\Cref{fig:EnvDesign} for a selection of different stages of the environment design). With the environment being a crucial part of the success of the installation, we had to make sure that it allowed the cats enough agency to prioritise their well being by, e.g., allowing for full withdrawal from the robot into dens providing privacy or by providing multiple food stations and litter boxes, thereby minimising resource based conflict between cats. 

...
...

The design of the robot world, beyond the emphasis on the robot interaction, is a multi-faceted endeavour as a wide range of view-points need to be considered. 


\hl{https://dl.acm.org/doi/abs/10.1145/3544549.3582734}.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/Environment_design_V2.png}
    \caption{Various iterations (to be read from top left to bottom right), from initial inspiration by the art of Verner Panton, to 3d renderings and scale models, to the final full sized installation.}
    \label{fig:EnvDesign}
\end{figure*}
\begin{comment}
    



Following the environment, the robot posed a constant negotiation of contrasting interests and focus points depending on whose point-of-view was prioritised, e.g., the audience, the cats, or the artists. The final goal during the design and implementation of the robots movement followed the following mantra:
\begin{quote}
    \textit{``Design the robots movements in order to allow us to keep the cats engaged in a safe, but non-boring, way.''}
\end{quote}

The cats, being unaware of the audience and the artists interests, this meant their only priority was the perfect balance between predictable routine and exciting novelty which in itself posed a significant challenge.

From the artists point of view, this meant making sure that 

the movements had to be designed and implemented in a way that was at the same time engaging for the cats, aesthetic for audience, as well as capable of expressing the artistic vision. 

We want to design to keep the cats engaged in a safe, but non-boring, way 

three primary stakeholders:
need movements to express what the artists want to express
need movements that are executable within given the specific robot affordances
need movements that can be executed without endangering the cats

\hl{Notes:} 
\begin{itemize}
    \item Quick description of: How were robot movements created.
    \item The robot movements had to be controlled and slow enough to guarantee cat safety, while being explosive and varied enough to be engaging for both cats and therefore for the audience.
\end{itemize}


\begin{quote}
    \textit{``The robot is competing [for the cats' attention] with the environment.''} - ACI specialist on team

    \textit{``The current playtime duration ( 1--4 minutes) is actually really good for a cat''} - Veterinarian on team
\end{quote}


\subsubsection{End-effectors and Toys}
\hl{Notes:} 
\begin{itemize}
    \item The choice of expanding the robots capabilities by designing custom end-effectors which provide the cats, and the robot, with additional affordances significantly affecting the interaction.
    \item The importance of not only creating toys that engage the cats, but also toys that are visually attractive for the audience. An example is the fish or bird toy which might not remind the cats of an actual cat or fish, but look visually appealing for the audience.
\end{itemize}

String based tasks are less deterministic due to the randomness in placement before pick-up. This makes them harder to control.


\newpage
\subsubsection{The Environment}
Inpired by art the rounded shapes by art from the 70s, e.g., Verner Panton Visiona II exhibit, Cat Royale aimed at creating a cat utopia using organic shapes and colours. The environment went through numerous iterations, sketches, mock-ups, 3d renderings, physical scale models, until it arrived at the final installation (see~\Cref{fig:EnvDesign} for a selection of different stages of the environment design). With the environment being a crucial part of the success of the installation, we had to make sure that it allowed the cats enough agency to prioritise their well being by, e.g., allowing for full withdrawal from the robot into dens providing privacy... 


\hl{https://dl.acm.org/doi/abs/10.1145/3544549.3582734}.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/Environment_design_V2.png}
    \caption{Various iterations (to be read from top left to bottom right), from initial inspiration by the art of Verner Panton, to 3d renderings and scale models, to the final full sized installation.}
    \label{fig:EnvDesign}
\end{figure*}

\end{comment}

==> Sections/X_Stakeholders.tex <==
\subsection{Two Types of Stakeholders}\label{sec:TheActors}
While the project involved a multitude of different stakeholders before, during, and after its installation, the primary stakeholders can be divided into the two following distinct categories: human and non-human stakeholders. This section highlights the implications these stakeholders had, as well as how and why we used the focus on non-human stakeholders --- in addition to the standard human (only) stakeholders in HRI --- affected the evolution, design, and ethics of the project.

%This section will emphasise points of interest for the three primary actors of the Cat Royale project, specifically: The humans involved, the three cats, and the robot.

\subsubsection{Human stakeholders}
n line with ACI (Animal Computer Interaction) research recommendations~\cite{Mancini:ACI:2011}, the Cat Royale project placed the animals at the centre of the design process,  there were also a multitude of human stakeholders were involved and therefore had to be accounted for during the conceptualisation and deployment of the artistic installation. Most noticeably, the artists, the robot operator, and the audience \hl{(NOTE: Should we here mention the AWO, the toy wrangler, the cat owner, the vision mixer)}. While the human actors took up different roles, collaborating around the same tasks, i.e., to increase the cats happiness and successfully deliver an artistic installation to the audience while ensuring cat welfare, their impact on the installation varied. The audience had no direct impact on the execution of the project, however, they were involved in its conceptualisation --- represented by 15 members of the general public, forming the Audience Advisory Panel (AAP). Through this method of involvement, the general public (represented as a sample) was given a voice in the design of the project, there opinions were used as both a mechanism by which the artists could gauge the impact of the work, and also as a way for the artists to directly find out more about the public perception of the work . Behind the scenes of Cat Royale (see~\Cref{fig:ControlRoom} left) the artist and the robot operator engaged in close collaboration to ensure the success of these two points, this co-ordination between artist and operator was key to the smooth running of the installation and decisions where made accordingly. Withint the workflow of the system, and specifically the decision engine part of the system,  as described in~\Cref{sec:TheCobot}, proposes actions for the robot to carry out in order to increase the happiness of the cats (according to the system). At this point the directing artist (who is seated next to the robot arm operator)  makes a judgement call --- to trust and accept the system's recommendation, executing the proposed action and hoping it leads to increased joy, ergo happiness for the cats and excitement for the audience, or to reject the proposed action and request a new one. The robot operator follows the decision of the artist, monitoring the robot during task execution. Their primary task was ensuring that the robot's percieved and in-actiion trajectory would not collide or in any other way endanger the cats. Therefore, the final control decision, at least behind the scenes was placed with the remit of the robot operator, as they could --- go against the artists and the decision engine's recommendation --- stop any robot action if they perceived it as posing a risk to the cats.

\begin{figure}[t]
    \centering
    %For cats_por_v1, height 3.3
    \includegraphics[height=3.75cm]{Figures/ControlRoom.jpg}
    \includegraphics[height=3.75cm]{Figures/Cats_Portrait_v2.png}
    \caption{\hl{This will be one part of a collage. Faces will be blurred.}}
    \label{fig:ControlRoom}
\end{figure}



\subsubsection{Non-human Stakeholders}
In contrast to the \hl{majority} of HRI research, which predominantly focuses upon humans, our system's 'users' were companion animals,  these were at thecentre of the design process. In many respects the role of humans in the system was secondary, at some points the robot arm and its existence in the system was also prioritised - possible due to the nature of the engagement between cat and robot arm. As non-human stakeholders (such as cats) are increasingly encountering autonomous systems, and vice-versa, it is important to understand how we design for, and with, non-human stakeholders. The Cats' involvement was an ongoing process, which ranged from recruitment of the specific animals, i.e., Clover, Pumpkin, and Ghostbuster (see~\Cref{fig:ControlRoom}, left to right), to assessing their wellbing during the sessions they were with the robot arm, their owner was with them throughout the whole period, and  following the conclusion of the installation actions were taken to see if they were OK. 

The welfare of the animals was a  priority, animal recruitment was vital prior to deployment of Cat Royale. The cats not only needed to be familiar with each other, but also within close proximity of the art studio in which the environment was to be built. These criteria were informed through consultation of feline behaviourists. Both aspects were vital in order to reduce the potential stress linked to meeting new cats, as well as in relation to the transport required, too much transport can disrupt a cat and mke it unhappy. Furthermore, in order to make sure that the cats were not deprived of contact to their owner, the cat recruitment relied on an owner who would be able to move into the art studio for \hl{17 days}, twelve days of deployment and five additional days during the habituation period prior to the deployment.
In addition to this there were design issues relating to aspects of cat proximity, which impacted upon the  cat's temperament as well as visual features. Three visually distinct cats were chosen to improve the reliability and ease of computational vision required for the recognition of the individual cats, this was a factor that needed to be considered relating to  the ease of detection for the underlying CV system. If the cats looked to similar the system would not be able to distinguish between them , and the decision engine would not be able to make decisions for a specific cat.
In line with Mancini's~\cite{Mancini:ACI:2011} Animal-Computer Interaction manifesto we made sure that we acquired two different types of consent from the feline participants. Firstly, we ensured consent from the cat owner, and secondly by designing the environment and the robot (as well as its placement) in a way that allows the cats to withdraw their contingent consent, by choosing not to engage with the robot.  The environment was designed to allow the cats to withdraw into their own space, as some occasionally did.

\begin{quote}
    \hl{Note:} \textit{Does the cat know what is best for it? Maybe what it wants is not what it needs?}
\end{quote}


==> Sections/X_Study.tex <==
\section{Cat Royale}
To investigate multispecies interaction with a (semi)autonomous system, the Cat Royale project team, comprising artists and a multidisciplinary set of researchers, asked itself the following question:
\begin{quote}
    \textit{``How do we situate an autonomous system within a wider environment, which is simultaneously engaging for spectators, ensures cat well-being, and is suitable for the autonomous system to operate in?''}
\end{quote}

%To investigate this multi-species interaction with a (semi)autonomous system, we used the artist-led Cat Royale project. 
This section will briefly outline the project, its three key actors, as well as its setting. A simplified version of the key components and actors of the Cat Royale project can be seen in~\Cref{fig:CRSystem}.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/System.png}
    \caption{\hl{Not sure we need an illustration like this (or the evolving one I presented at the TAS AHM) to showcase the relationship between the four main components}, i.e., \textit{a selection of human stakeholders (yellow), non-human stakeholders (green), the robotic system (red)}, and the \textit{robot world (blue box)}.}
    \label{fig:CRSystem}
\end{figure}


%The project introduction, and the need for it, is inspired by the aci paper.
\subsection{Cat Royale: The Artistic Installation}
The design process of Cat Royale, which this paper will focus on, was developed over the course of eighteen months. 
The centrepiece was a bespoke environment, built for and inhabited by three cats. The cats, a parent and two offspring, spent six hours a day (two periods of three hours) over twelve consecutive days within the environment, a total of 72 hours. Cat Royale attempted to be a utopia for cats, by catering to the cats' various needs including appropriate spaces, dens, perches, walkways, feeding areas, cat friendly plants, and litter trays. Waiting in the centre of the room was the robotic arm, ready to identify and fulfil every playful desire of Ghostbuster, Clover, and Pumpkin, the three inhabitants of the environment. Provided with access to a series of custom end-effectors and a wide range of different toys and attachments, both for play and for snack time, the robot waited to spring into action at a moment's notice. At regular intervals, the robots underlying AI system proposed a robot action aimed at maximising a specific cat's assessed happiness. If approved by the creative minds behind the installation, the robot would execute a playful activity aimed at increasing the cats' happiness, while being monitored by the robot operator to ensure safe robot movement in close proximity to the cats. To further ensure animal welfare, each cat's individual stress score~\cite{kessler:turner:1997} was ranked at 15-minute intervals by the team's specialist in feline behaviour. The robot performed more than 500 activities over the course of the 12 days, ranging from providing small cat treats\footnote{Regular food and water was available to the cats at all times, regardless of their engagement with the robot.}, to simple things like a cardbox or a string, all the way to more elaborate toys such as an orange bird toy or a battery powered wiggling fish toy. Following each activity, each cat's engagement---as a proxy for positive attitude towards the robot-provided entertainment---was ranked using the Participation in Play scale~\cite{Ellis:2022:Pip}, a tool typically used in cat behaviour studies to assess engagement in playful activities. The task executed (i.e., `present a prey game with a toy bird'), the targeted cat, as well as the impact on happiness where consecutively fed back into the robots machine learning system (i.e., the decision engine) informing future proposed activities. 

All cat and robot activities within the environment were constantly filmed using eight cameras, the output of which was mixed by an experienced television vision mixer to produce the six-hour long daily film shown to public audiences at the Curiocity Brisbane World Science Festival. Furthermore, the entire 572 hours of footage (6 hours $\times$ 8 cameras $\times$ 12 days) was edited into an 8 hour highlight movie which is currently at display at the National Science Gallery in London\footnote{https://london.sciencegallery.com/ai-artworks/cat-royale}. Lastly, daily highlight videos (2 -- 5 minutes) were edited and showcased online.

The environment was aiming not only to provide the cats with everything they could possibly desire but also to provoke questions among the audience. `What is a Cat utopia?', `Can AI even detect animal (or human) happiness?', and `Is it beneficial to have every desire fulfilled at a moment's notice?' are examples of such questions.

%The environment was constantly filmed using eight cameras, whose outputs were mixed by an experienced television vision mixer to produce video material to be edited and later shown to public audiences in a gallery during a prestigious Art and Science festival, and a short daily highlight video for social media. As a result, the public audience watched the cats’ experience of the robot as a video installation that could readily tour to multiple galleries worldwide. 

%%%%%%%%%%%%


%To investigate multi-species interaction with (semi)autonomous systems, we used the artist-led Cat Royale project. Its involvement of different stakeholders and actors allowed us to investigate multi-species design a bespoke environment while being in constant negotiation between different actors in the ecology. In addition to the actors involved, we designed and developed the physical setting for this artistic installation. This section will describe the different perspectives, i.e., cats, robot, and humans, and highlight their respective focus points impacting the design of Cat Royale as multi-species environment. 

\input{Sections/_Stakeholders}
\input{Sections/_RobotAndWorld}
